NLTS Hamiltonians from good quantum codes

The NLTS (No Low-Energy Trivial State) conjecture of Freedman and Hastings [2014] posits that there exist families of Hamiltonians with all low energy states of non-trivial complexity (with complexity measured by the quantum circuit depth preparing the state). We prove this conjecture by showing that the recently discovered families of constant-rate and linear-distance QLDPC codes correspond to NLTS local Hamiltonians.

==> berkeleymacros.tex <==
%% Useful Extra Packages

\usepackage{graphicx, subfigure}
\usepackage{enumitem}
\usepackage{xparse}
\usepackage{physics}
\usepackage{color}


%% Bold Letters

\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\B}{\mathbf{B}}
% \newcommand{\E}{\mathbf{E}}


%% Blackboard Letters

\newcommand{\CC}{\mathbb{C}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\ZZ}{\mathbb{Z}}

%% Caligraphy Letters

\newcommand{\Aa}{\mathcal{A}}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dd}{\mathcal{D}}
\newcommand{\Ff}{\mathcal{F}}
\newcommand{\Gg}{\mathcal{G}}
\newcommand{\Hh}{\mathcal{H}}
\newcommand{\Ll}{\mathcal{L}}
\newcommand{\Mm}{\mathcal{M}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Oo}{\mathcal{O}}
\newcommand{\Pp}{\mathcal{P}}
\newcommand{\Rr}{\mathcal{R}}
\newcommand{\Qq}{\mathcal{Q}}
\newcommand{\Ss}{\mathcal{S}}
\newcommand{\Tt}{\mathcal{T}}
\newcommand{\Uu}{\mathcal{U}}
\newcommand{\Xx}{\mathcal{X}}
\newcommand{\Yy}{\mathcal{Y}}

\newcommand{\X}{\mathsf{x}}
\newcommand{\Z}{ \mathsf{z}}
\renewcommand{\H}{\mathbf{H}}

%% Classic Functions

\newcommand{\One}{\mathbf{1}}

\newcommand{\rnk}{\mathop{\mathbf{rnk}\hspace{0.05em}}}
\newcommand{\Exp}{\mathop{\mathbf{E}\hspace{0.13em}}}

\newcommand{\Var}{\mathop{\mathbf{Var}\hspace{0.13em}}}
\newcommand{\inv}[1]{#1^{-1}}
\newcommand{\realp}{\mathfrak{Re}}
\newcommand{\imagp}{\mathfrak{Im}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\negl}{\mathrm{negl}}
% \newcommand{\poly}{\mathrm{poly}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\range}{\mathrm{range}}
\newcommand{\dom}{\mathrm{dom}}
% \newcommand{\supp}{\mathrm{supp}}
\newcommand{\sgn}{\mathrm{sgn}}
\renewcommand{\Pr}{\mathop{\mathbf{Pr}\hspace{0.05em}}}

\newcommand{\argmax}{\mathop{\mathrm{argmax\hspace{0.05em}}}}

\newcommand{\Id}{\mathbb{1}}

%% Shortcuts to Phrases

\newcommand{\eps}{\epsilon}
\newcommand{\true}{\mathsf{True}}
\newcommand{\false}{\mathsf{False}}
\newcommand{\nil}{\mathsf{null}}
\newcommand{\st}{\text{ s.t. }}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\pf}{\mathsf{pf}}

%% Equality Symbols

\newcommand{\defeq}{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily def}}}{=}}}

\newcommand{\intersect}{{\ni\joinrel\in}}
\newcommand{\disjoint}{\centernot{\intersect}}

%% Complexity Classes
\usepackage{complexity}
\newcommand{\SHARPP}{\mathsf{\#}\P}
\newcommand{\PZKMIP}{\mathsf{PZKMIP}}

\renewcommand{\exp}{\mathsf{exp}}

%% Classic Problems
\newcommand{\maxcut}{\textsc{maxcut}}
\newcommand{\gw}{\textsc{gw}}

%% Other Theoretical CS Phrases

\newcommand{\OPT}{\textbf{OPT}}
\newcommand{\bits}{\{0,1\}}

%% Special Propositions

\newcommand{\specialprop}[2]{
   \newtheorem*{thm#1}{Proposition #1}\begin{thm#1}#2\end{thm#1}}

%% Repeated Statements

\newcommand{\fn}[3]{#1: #2 \rightarrow #3}
\newcommand{\bitsfn}[3]{\fn{#1}{\bits^{#2}}{\bits^{#3}}}

%% Cryptography

\newcommand{\owff}{\Ff = \{\bitsfn{f_k}{n(k)}{m(k)}\}_k}

\newcommand{\PK}{\mathsf{PK}}
\newcommand{\SK}{\mathsf{SK}}

\newcommand{\Enc}{\mathtt{Enc}}
\newcommand{\Dec}{\mathtt{Dec}}

% Quantum

\newcommand{\EPR}{\mathrm{EPR}}
\newcommand{\cat}{\mathsf{cat}}
\newcommand{\NLETS}{\mathsf{NLETS}}
\newcommand{\NLTS}{\mathsf{NLTS}}
\newcommand{\qPCP}{\mathsf{qPCP}}
\newcommand{\LH}{\mathsf{LH}}

\newcommand{\junk}{\mathsf{junk}}
\newcommand{\unary}{\mathsf{unary}}
\newcommand{\state}{\mathsf{state}}
\newcommand{\ancilla}{\mathsf{ancilla}}

\newcommand{\qudit}[1]{\CC^{#1}}
\newcommand{\qudits}[2]{(\qudit{#1})^{\otimes #2}}

\newcommand{\qubit}{\CC^{2}}
\newcommand{\qubits}[1]{(\qubit)^{\otimes #1}}

\newcommand{\Cliff}{\mathsf{Cliff}}

\newcommand{\QCSAT}{\mathrm{QCSAT}}

% gates

\newcommand{\CNOT}{\mathrm{CNOT}}


\newcommand{\unsat}{\mathrm{unsat}}
\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}

\newcommand{\eff}{\mathsf{eff}}

\newcommand{\yes}{\mathsf{yes}}
\newcommand{\no}{\mathsf{no}}


\renewcommand{\eqref}[1]{\textrm{eq.~}(\ref{#1})}

\newcommand{\YES}{\mathsf{YES}}
\newcommand{\NO}{\mathsf{NO}}

\renewcommand{\exp}{\mathrm{exp}}
